Amortized Probabilistic Conditioning for Optimization, Simulation and Inference

Amortized meta-learning methods based on pre-training have propelled fields like natural language processing and vision. Transformer-based neural processes and their variants are leading models for probabilistic meta-learning with a tractable objective. Often trained on synthetic data, these models implicitly capture essential latent information in the data-generation process. However, existing methods do not allow users to flexibly inject (condition on) and extract (predict) this probabilistic latent information at runtime, which is key to many tasks. We introduce the Amortized Conditioning Engine (ACE), a new transformer-based meta-learning model that explicitly represents latent variables of interest. ACE affords conditioning on both observed data and interpretable latent variables, the inclusion of priors at runtime, and outputs predictive distributions for discrete and continuous data and latents. We show ACE's modeling flexibility and performance in diverse tasks such as image completion and classification, Bayesian optimization, and simulation-based inference.

==> image_files/celeba_nlpd.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
axis on top,
enlarge x limits=false,
enlarge y limits=false,
    height=\figureheight,
    width=\figurewidth,
    tick align=outside,
    tick pos=left,
    x grid style={white!69.0196078431373!black},
    %ylabel={Negative Log Predictive Density},
    xmajorgrids,
    ymajorgrids,
    ylabel near ticks,
    xmin=4, xmax=26,
    ymin=-1.15828497707844, ymax=0.514319315552711,
    xtick style={color=black},
    ytick style={color=black},
    % Add a % symbol to the x-axis tick labels
    xticklabel={\pgfmathprintnumber{\tick}\%},
    % Set smaller font for axis numbers
    tick label style={font=\tiny},
    % Set smaller font for axis labels
    label style={font=\tiny},
]
\addplot [semithick, color0, mark=*, mark size=2, mark options={solid}]
table {%
5 -0.264539301395416
10 -0.567088305950165
15 -0.774066746234894
20 -0.916227519512177
25 -1.07542681694031
};
\addplot [semithick, color1, mark=*, mark size=2, mark options={solid}]
table {%
5 -0.286855936050415
10 -0.580686688423157
15 -0.784428417682648
20 -0.92386931180954
25 -1.08225750923157
};
\addplot [semithick, color2, mark=*, mark size=2, mark options={solid}]
table {%
5 0.438291847705841
10 0.102120257914066
15 -0.114910803735256
20 -0.282689064741135
25 -0.427615821361542
};
\end{axis}

\end{tikzpicture}


==> image_files/mnist_nlpd.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
height=\figureheight,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={white!69.0196078431373!black},
%xlabel={Context Size (\% of Image)},
xmin=-1.85, xmax=60.85,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={NLPD},
ymin=-1.77795943521061, ymax=-0.349201389574808,
ytick style={color=black}
]
\path [fill=color0, fill opacity=0.2]
(axis cs:1,-0.616825573991267)
--(axis cs:1,-0.891079009224446)
--(axis cs:3,-1.02534877095046)
--(axis cs:7,-1.04066708014128)
--(axis cs:11,-1.12720083510309)
--(axis cs:15,-1.21576526108963)
--(axis cs:19,-1.31270018464268)
--(axis cs:23,-1.33954204540862)
--(axis cs:27,-1.39115316667803)
--(axis cs:39,-1.5094871845793)
--(axis cs:58,-1.61613726554564)
--(axis cs:58,-1.44500006498643)
--(axis cs:58,-1.44500006498643)
--(axis cs:39,-1.29792714447267)
--(axis cs:27,-1.19506551227324)
--(axis cs:23,-1.1626264907776)
--(axis cs:19,-1.09038336628735)
--(axis cs:15,-1.00993632134217)
--(axis cs:11,-0.870729518776835)
--(axis cs:7,-0.771025652431273)
--(axis cs:3,-0.626550358201834)
--(axis cs:1,-0.616825573991267)
--cycle;

\path [fill=color1, fill opacity=0.2]
(axis cs:1,-1.10294341069542)
--(axis cs:1,-1.29446497934974)
--(axis cs:3,-1.35994081138584)
--(axis cs:7,-1.43890222752126)
--(axis cs:11,-1.47455791625467)
--(axis cs:15,-1.54272788035915)
--(axis cs:19,-1.5782706855719)
--(axis cs:23,-1.58192795260562)
--(axis cs:27,-1.60207163191102)
--(axis cs:39,-1.65084946778611)
--(axis cs:58,-1.71301588768171)
--(axis cs:58,-1.61638604646517)
--(axis cs:58,-1.61638604646517)
--(axis cs:39,-1.55480005118057)
--(axis cs:27,-1.51440440320709)
--(axis cs:23,-1.5029783631979)
--(axis cs:19,-1.45578261623931)
--(axis cs:15,-1.40164074432804)
--(axis cs:11,-1.35351798143896)
--(axis cs:7,-1.28319662368266)
--(axis cs:3,-1.18714079023388)
--(axis cs:1,-1.10294341069542)
--cycle;

\path [fill=color2, fill opacity=0.2]
(axis cs:1,-0.414144937103708)
--(axis cs:1,-0.565075944954436)
--(axis cs:3,-0.639225034745033)
--(axis cs:7,-0.728249123589601)
--(axis cs:11,-0.804179363927266)
--(axis cs:15,-0.882780949124098)
--(axis cs:19,-0.933400161560369)
--(axis cs:23,-0.958819397721978)
--(axis cs:27,-0.980248094461341)
--(axis cs:39,-1.0286754745553)
--(axis cs:58,-1.06856436944198)
--(axis cs:58,-0.999594996212013)
--(axis cs:58,-0.999594996212013)
--(axis cs:39,-0.957081059782702)
--(axis cs:27,-0.904474233724694)
--(axis cs:23,-0.88277557250431)
--(axis cs:19,-0.821323685352015)
--(axis cs:15,-0.776103939763307)
--(axis cs:11,-0.698159736910442)
--(axis cs:7,-0.617504194481764)
--(axis cs:3,-0.486283854810898)
--(axis cs:1,-0.414144937103708)
--cycle;

\addplot [semithick, color0, mark=*, mark size=3, mark options={solid}]
table {%
1 -0.753952291607857
3 -0.825949564576149
7 -0.905846366286278
11 -0.998965176939964
15 -1.1128507912159
19 -1.20154177546501
23 -1.25108426809311
27 -1.29310933947563
39 -1.40370716452599
58 -1.53056866526604
};
\addlegendentry{\tiny{ACE no conditioning}}
\addplot [semithick, color1, mark=*, mark size=3, mark options={solid}]
table {%
1 -1.19870419502258
3 -1.27354080080986
7 -1.36104942560196
11 -1.41403794884682
15 -1.4721843123436
19 -1.51702665090561
23 -1.54245315790176
27 -1.55823801755905
39 -1.60282475948334
58 -1.66470096707344
};
\addlegendentry{\tiny{ACE conditioned class}}
\addplot [semithick, color2, mark=*, mark size=3, mark options={solid}]
table {%
1 -0.489610441029072
3 -0.562754444777966
7 -0.672876659035683
11 -0.751169550418854
15 -0.829442444443703
19 -0.877361923456192
23 -0.920797485113144
27 -0.942361164093018
39 -0.992878267168999
58 -1.034079682827
};
\addlegendentry{\tiny{TNPD}}
\end{axis}

\end{tikzpicture}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> misc.tex <==
\section{Ideas}
%\subsection*{Data and Latent Representation}

%We represent data points as tuples (data type, covariate, value), e.g. $(0, \x, y)$:

%\begin{itemize}
%\item \emph{Data type} for the moment can be 0 for `data' and $1$ for `latent'. 
%\item For the data, the \emph{covariate} $\x \in \mathbb{R}^D$ is a continuous vector in $D \ge 0$ dimensions. For the latents, the covariate is an integer $1 \le k \le K$ denoting the latent index (latents belong to a discrete set). For example, for the optimization task, the latents will be $(\mathbf{x}_1^{\text{opt}}, \mathbf{x}_2^{\text{opt}}, \ldots, \mathbf{x}_D^{\text{opt}}, y^{\text{opt}})$ and $K = D + 1$.
%\item The \emph{value} $y \in \mathbb{R}$ is generally assumed to be a scalar. This is not limiting: multi-output values can be expressed by adding an extra index in the covariate specifying the output dimensions, e.g. for a $M$-valued output we would have $(0, (\x, m), y_m)$, for $1 \le m \le M$.
%To denote a `padded value', $y$ is replaced by $?$ in a target point before being fed to the network (the true target $y$ is used for evaluating the log likelihood of the predictions).
%\end{itemize}


\subsubsection*{Embeddings}

\begin{itemize}
\item We embed context data points $(\x, y)$ to $\mathbb{R}^{N_\text{rep}}$ as $f_\text{cov}(\x) \oplus f_\text{val}(y)$ where the sum can be just vector sum or concatenation (ideally standard vector sum is fine and the Transformer will figure out what to do with it). $f_\text{cov}$ and $f_\text{val}$ are two nonlinear embeddings (MLPs) for covariates and values, respectively.
\item We embed context latents $(k, y)$ using a discrete embedding $E_k$ for the $k$-th latent (i.e., $k$-th row of a learnt embedding latent matrix). The full embedding is $E_k \oplus f_\text{val}(y)$.\footnote{It might be useful here to add a learnt $E_\text{latent}$ vector to all latent embeddings, but 
 for the moment I did not include it.}
\item For target data or latents, $f_\text{val}(?)$ is directly replaced with $E_?$, a learnt vector embedding for the $?$ symbol.
\item The general idea above is that anything that is continuous has a nonlinear embedding; everything discrete (out of a finite set) just directly maps to a learnt embedding vector.
\item The representation above does not explicitly force $f_\text{cov}(\x)$ to differ from $E_k$, meaning that accidentally a data embedding might look like a latent embedding. However, let's see if this is actually a problem. In principle the network should automatically learn to ensure that the two types of embeddings are well separated.
\end{itemize}

\subsection{General}

\paragraph{Main idea.}
Use (transformer, conditional) neural processes, or similar other CNP architectures like the ones we described, to learn both posteriors over latent variables and predictive distributions over data in a variety of tasks. The idea is to extend the way we handle data points in a T/CNP by explicitly adding ``latent variables''. Then ideally we can change the task elegantly by just moving the data and latents to the context set and/or target set (if in the context set, we are conditioning over data and latents; if in the target set, we are predicting latents, aka posteriors, and data, aka posterior predictive). Note that the point is not to outperform existing NP models, but to show a new application for them.

\paragraph{Applications.}
In terms of tasks, we would showcase some examples in:
\begin{itemize}
\item Simulator-based inference (latents are model parameters);
\item Optimization (latents are location and value of the optimum, maybe something else like features of the function);
\item Possibly another task to be thought of.
\end{itemize}

\paragraph{Scope.}
Presumably in this paper we do the following things (open to discussion):
\begin{itemize}
\item We train each NP on a single (or small) model class, e.g. one simulator model, one or a few GP kernels, like in previous NP papers. We are not aiming for big meta-learning across huge model classes (which is going to be the goal for the Large Inference Model paper).
\item We focus on continuous data and latents, but we may want to include some examples with discrete data/latents since it shouldn't be too hard to add and it's e.g. something that our architecture can deal with easily as opposed to normalizing flows. We will treat discrete variables in a simple manner (e.g., one-hot encoding, simple tokenization; nothing like a grammar).
\item We can probably assume a fixed number of parameters $D$ for the model being trained, like in the other NP papers. We don't strictly need to tackle variable-dimension and feature-equivariance in this paper. However, this is up for discussion (e.g., the optimization examples would look better if we don't need to train a separate NP for each $D$).
\item We will compare a few \emph{*NP} architectures (plus some new \emph{*NP} architecture we can come up with), since the core paper idea is pretty much orthogonal to the implementation.
\item Since we have both data and latents to predict, and they could be both continuous and discrete, for the moment the only way we can do that scalably is autoregressively - i.e. at inference time we predict the target set autoregressively (which might require Monte Carlo sampling to manually permute the order of the target set). In training, this means that (unless we use some tricks), if we present a target set, we are treating the elements of the target set independently as parallel predictions.
\end{itemize}

\subsection{Other points}
 
\paragraph{Conditional Predictive Distributions.}
\begin{itemize}
    \item We have settled to use a mixture density (e.g., a mixture of Gaussians), like in this paper: \url{https://arxiv.org/abs/1605.02226}
    \item One unsolved thing is how to deal with $p(\mathbf{y}^\star|\mathbf{x}^\star,\text{rest of the context})$ when the values we care about are multidimensional. One answer as we have done so far is `autoregressively' but this doesn’t quite work in all the cases. For example Daolang
 correctly remarked that at least in some cases we may have $\mathbf{y}$ without $\mathbf{x}$. In that case it’s not obvious how to predict a multidimensional $\mathbf{y}$ autoregressively. I don’t mean many distinct datapoints but a single datapoint with many output features.
 One solution may be to go with a mixture of Gaussians in $d_\text{output}$ dimensions.
\end{itemize}

\paragraph{Batch Context Training}

\begin{itemize}
\item The standard TCNP architecture does not afford efficient `batch context' training. Given a context set $(\textbf{X}, \textbf{Y})$, any change to the context (e.g., adding one point) corresponds to a completely different training instance.
\item An architecture with \emph{independent encoding} of the context points, instead, affords batch context training. To do so, duplicate the target set along the batch dimension, and then apply masking to the attention matrix from target to the context, where the masking represents different subsets of the context (with and without latents). 
\item The masking needs to be built smartly: e.g. for each row in the mask matrix, sample $N_\text{context}$ uniformly from $N_\text{min}$ to $N_\text{max}$, and these are the unmasked data points (chosen randomly inside the context set); then there is some probability $p$ that there are no latents (e.g., $p = 0.5$); if there are latents, draw uniformly randomly from 1 to $N_\text{latents}$ the number of latents to unmask, and pick them randomly.
\item Be sure to mask things correctly such that if a latent is present (unmasked) in the context, it is \emph{removed} form the corresponding target set (or at least it should not contribute to the loss).
\end{itemize}



\section{Architectures}

\subsection{Transformer CNP}

The baseline architecture we are considering is (a small variant of) the Transformer Conditional Neural Process, or TCNP. 

\begin{figure} 
\centering
\[
    \begin{array}{r}
 \text{register} \\
 \\
 \\
 \text{context} \\
 \\
 \text{target} \\
 \\
\end{array}
\begin{bmatrix}
    \begin{array}{c|c|c}
        \begin{matrix}
            1 & 1 \\
            1 & 1
        \end{matrix} & \begin{matrix}
            1 & 1 & 1 \\
            1 & 1 & 1
        \end{matrix} & \begin{matrix}
            0 & 0 \\
            0 & 0
        \end{matrix} \\ \hline
        \begin{matrix}
            0 & 0 \\
            0 & 0 \\
            0 & 0
        \end{matrix} & \begin{matrix}
            1 & 0 & 0 \\
            0 & 1 & 0 \\
            0 & 0 & 1
        \end{matrix} & \begin{matrix}
            0 & 0 \\
            0 & 0 \\
            0 & 0
        \end{matrix} \\ \hline
        \begin{matrix}
            1 & 1 \\
            1 & 1
        \end{matrix} & \begin{matrix}
            1 & 1 & 1 \\
            1 & 1 & 1
        \end{matrix} & \begin{matrix}
            1 & 0 \\
            0 & 1
        \end{matrix}
    \end{array}
\end{bmatrix}
\]
\hspace{0.4cm}
\makebox[35pt][l]{$\underbrace{\hspace{1cm}}_{\text{register}}$}
\makebox[50pt][l]{$\underbrace{\hspace{1.4cm}}_{\text{context}}$}
\makebox[0pt][l]{$\underbrace{\hspace{1cm}}_{\text{target}}$}
\label{fig:tcnp_reg_mask}
\caption{Attention mask for the independent-encoder TCNP with register. Note that the register fully attends to itself and to the context. The context points remain independent of everything. Each target points attends to the context and to the register, independently of other targets. This is an illustrative diagram; in practice this would not be implemented with a full matrix.}
\end{figure}

The general idea of the TCNP is, assuming the diagonal TCNP:
\begin{itemize}
\item \emph{Context} points are passed through a `fully connected' transformer with full self-attention.
\item At the same time, the \emph{target} data points attend each one to itself\footnote{Actually, I realized later that this is not the case for the TCNP paper; see Section \ref{sec:selfselfattention}.} and to all the points of the context set. %(This is similar but not fully identical to cross-attention because cross attention does not include the current point.)
\item Context and targets are processed in tandem, with $N_\text{blocks}$ stacked transformer blocks each.
\item The attention mask is represented in Figure \ref{fig:tcnp_mask}. This mask is applied elementwise to the attention weights matrix.\footnote{In practice, you would replace the log weights where the mask is 0 with \texttt{-Inf} \emph{before} computing the softmax, so that the attention weight at $A_{n,n^\prime}$ is zero where the mask is zero.}
\end{itemize}

\begin{figure} \label{fig:tcnp_mask}
    \centering
\[
\begin{array}{r}
 \\
 \text{context} \\
 \\
 \text{target} \\
 \\
\end{array}
\begin{bmatrix}
    \begin{array}{c|c}
        \begin{matrix}
            1 & 1 & 1 \\
            1 & 1 & 1 \\
            1 & 1 & 1
        \end{matrix} & \begin{matrix}
            0 & 0 \\
            0 & 0 \\
            0 & 0
        \end{matrix} \\ \hline
        \begin{matrix}
            1 & 1 & 1 \\
            1 & 1 & 1 \\
        \end{matrix} & \begin{matrix}
            1 & 0 \\
            0 & 1
        \end{matrix}
    \end{array}
\end{bmatrix}
\]
\hspace{0.4cm}
\makebox[50pt][l]{$\underbrace{\hspace{1.5cm}}_{\text{context}}$}
\makebox[0pt][l]{$\underbrace{\hspace{1cm}}_{\text{target}}$}
\caption{Attention mask for the standard TCNP. The context text fully attends to the context set, but not to the target. Each element of the target separately attends to each element of the context set, but not to other targets. This is an illustrative diagram; in practice this would not be implemented with a full matrix.}
\end{figure}

\textbf{Remarks:}
\begin{itemize}
\item The architecture above means that we are treating the target points in parallel, so we want to always add as many data points (and all latents) to the target set when training. As far as I can see, there is \emph{no reason} for not training on a target set as large as whatever we can fit in memory (for the current batch).
\item As we discussed several times, the fact that the context set is fully connected means that we cannot reuse computations: if we add or remove a point from the context, that counts as a completely different training example.
\item The fact that context and target are processed at the same time means that in the current implementation if we decide to add a new target later we would need to re-process the context set. This is not fully true in that we could cache the intermediate layers of the context (since the context does not depend on the target), and pass these to future target computations -- as long as we don't change the context set.
\end{itemize}

The architectures below can be considered as variants that alter some aspects of encoding or decoding.


\subsection{Encoder}

By encoder we mean the neural network that deals with the context set, eventually encoding each context data point into a $N_\text{rep}$ dimensional representation. This is an encoder because it is building a representation of the context which does not depend on the target, although in the TCNP encoder (context) and decoder (targets) are operating at the same time, but this is purely for convenience. As mentioned above, we could cache the intermediate steps of the encoder (the outputs of each transformer block) and first encode the context and then separately decode it on the targets.

I will call `independent' an encoder in which all data points are encoded independently of each other.

\begin{itemize}
\item As described above, the default TCNP encoder is a series of fully connected transformer blocks. This encoder is \emph{not} independent.
\item A basic \emph{independent} encoder is a MLP applied separately in parallel to all context data points. A simple example is the CNP encoder (without summing at the end).
\begin{itemize}
    \item If we want this encoder to work together with the decoder, we may way want this MLP to be structured in $N_\text{block}$ blocks (each one with possibly multiple hidden layers). The input of each MLP block needs to be of size $N_\text{rep}$, and this is the input also fed to each stacked block of the decoder.
\end{itemize}
\item Another \emph{independent} encoder is a stack of $N_\text{blocks}$ transformer blocks with diagonal attention.\footnote{We actually would not calculate the attention matrix here as there is no need; the matrix is the identity.}
This differs from the previous option in that a transformer block is not just a MLP block, but has a few additional `niceties' (e.g., TokenNorm and residual connections\footnote{See Turner (2023), \url{https://arxiv.org/abs/2304.10557}.}). See Fig \ref{fig:diag_tcnp_mask}.
\end{itemize}

\begin{figure} \label{fig:diag_tcnp_mask}
    \centering
\[
\begin{array}{r}
 \\
 \text{context} \\
 \\
 \text{target} \\
 \\
\end{array}
\begin{bmatrix}
    \begin{array}{c|c}
        \begin{matrix}
            1 & 0 & 0 \\
            0 & 1 & 0 \\
            0 & 0 & 1
        \end{matrix} & \begin{matrix}
            0 & 0 \\
            0 & 0 \\
            0 & 0
        \end{matrix} \\ \hline
        \begin{matrix}
            1 & 1 & 1 \\
            1 & 1 & 1 \\
        \end{matrix} & \begin{matrix}
            1 & 0 \\
            0 & 1
        \end{matrix}
    \end{array}
\end{bmatrix}
\]
\hspace{0.4cm}
\makebox[50pt][l]{$\underbrace{\hspace{1.5cm}}_{\text{context}}$}
\makebox[0pt][l]{$\underbrace{\hspace{1cm}}_{\text{target}}$}
\caption{Attention mask for the independent-encoder TCNP. Here each context point does not talk to other context points. This is an illustrative diagram; in practice this would not be implemented with a full matrix.}
\end{figure}


\subsubsection{Register data}

As a part of the encoding process we can also optionally have $N_\text{reg}$ \emph{register} data points, also called memory or register tokens, inducing points, etc. In the standard TCNP $N_\text{reg} = 0$. An example with $N_\text{reg} = 1$ is the special \texttt{<cls>} token used in the Vision Transformer.\footnote{They are called `tokens' but these are for all effects additional (special) data points fed to the Transformer.}

In a nutshell, register points are special data points or tokens that are always given as input (in addition to the normal input data), and whose job is to explicitly provide the Transformer with an additional `global' computation scratchpad. This idea reappears in multiple ways in many papers. 
In our case, we are going to use the register to keep a global summary representation of the context.

This may be done in multiple ways but the ones I think we should explore are:
\begin{itemize}
\item The default of course is $N_\text{reg} = 0$ (no register).
\item The register has full self attention to itself, and also attends to all the context points (but the context does \emph{not} attend to the register).
\end{itemize}

A particularly interesting combination is having an \emph{independent} Transformer encoder with a register $N_\text{reg} > 0$. In this case, while it is true that individual context points do not directly talk to each other, there is still a global representation being built in the register. This has some of the advantages of keeping an independent context, while keeping \emph{some} ability for building a global representation.

\subsection{Decoder}

The decoder is a stack of Transformer blocks that maps target sets to their predictions (obtained at the last layer via a readout consisting of a mixture density, e.g. the parameters of a mixture of Gaussians).

\begin{itemize}
\item The standard solution is that each target point attends to itself and to the whole context.
\item If $N_\text{reg} > 0$ there are two main possible choices:
\begin{itemize}
\item Each target point attends to itself and to \emph{both} the context and the register, allowing the target to attend both to individual context points as well as to the global representation contained in the register. This is represented in Fig \ref{fig:tcnp_reg_mask}.
\item Each target point attends to itself and to the register but not directly to points in the context (this has better scaling but of course loses in granularity).
\end{itemize}
\end{itemize}

\subsection{Summary}

Just considering what has been listed above, there are several possible combinations  based on the encoder (at least three choices), the presence of register or not (two major choices; plus of course the choice of $N_\text{reg} > 0$ but that's an hyperparameter), and the type of decoder (no choice if $N_\text{reg} = 0$, two choices if $N_\text{reg} > 0$). We don't need to explore all possible combinations.

Particularly interesting combos for this paper are:
\begin{itemize}
\item TCNP (full Transformer encoder; no register; standard Transformer decoder); attention mask as in Fig \ref{fig:tcnp_mask}.
\item CNP-TCNP? (MLP encoder --- multilayer?; no register; standard TCNP decoder)
\item TCNP with diagonal encoder and register (diagonal Transformer encoder; no register; standard Transformer encoder); attention mask as in Fig \ref{fig:diag_tcnp_mask}.
\item TCNP with diagonal encoder and register (diagonal Transformer encoder; register with $N_\text{reg}>0$; Transformer encoder that attends to both register and context); attention mask as in Fig \ref{fig:tcnp_reg_mask}.
\end{itemize}

The CNP-TCNP and TCNP with diagonal encoder should afford efficient batch-ization of the context (i.e., learning multiple contexts from a single instance).
The same to a degree can be done also with the TCNP with diagonal encoder + register, with the care that for each subset of the context we also need to duplicate the register (but not the entire context set). I think this representation is promising on paper as it combines multiple desiderata (then whether it can be actually implemented efficiently, and whether it works in practice, are different questions...).

